Low-Frequency Stabilizations of the PMCHWT Equation for Dielectric and Conductive Media: On a Full-Wave Alternative to Eddy-Current Solvers

We propose here a novel stabilization strategy for the PMCHWT equation that cures its frequency and conductivity related instabilities and is obtained by leveraging quasi-Helmholtz projectors. The resulting formulation is well-conditioned in the entire low-frequency regime, including the eddy current one, and can be applied to arbitrarily penetrable materials, ranging from dielectric to conductive ones. In addition, by choosing the rescaling coefficients of the quasi-Helmholtz components appropriately, we prevent the typical loss of accuracy occurring at low frequency in the presence of inductive and capacitive type magnetic frill excitations, commonly used in circuit modeling to impose a potential difference. Finally, leveraging on quasi-Helmholtz projectors instead than on the standard Loop-Star decomposition, our formulation is also compatible with most fast solvers and is amenable to multiply connected geometries, without any computational overhead for the search for the global loops of the structure. The efficacy of the proposed preconditioning scheme when applied to both simply and multiply connected geometries is corroborated by numerical examples.

==> praemble/hft-macros-booktabs.tex <==
%% Booktabs

\newcolumntype {n}{c}
\newcolumntype {N}{>{\small}c}
\newcolumntype {L}{>{\small}l}
\newcolumntype {F}{>{\footnotesize}c}
\newcolumntype {v}[1]{>{\raggedright \hspace {0pt}} p {#1}}
\newcolumntype {V}[1]{>{\small \raggedright \hspace {0pt}} p {#1}}
\newcolumntype{d}[1]{>{\DC@{.}{.}{#1}}c<{\DC@end}}

\newcommand{\armultirow}[3]{%
    \multicolumn{#1}{#2}{%
        \begin{picture}(0,0)%
        \put(0,0){%
            \begin{tabular}[t]{@{}#2@{}}%
            #3%
            \end{tabular}%
        }%
        \end{picture}%
    }%
}%
% array.sty, rotating.sty
\newcolumntype{R}[1]{%
    >{\begin{turn}{90}\begin{minipage}{#1}\small\raggedright\hspace{0pt}}l%
            <{\end{minipage}\end{turn}}%
} 


==> praemble/hft-macros-environments.tex <==
\newcounter{subequation}
\newlength\mtabskip\mtabskip=-1.25cm
\renewcommand{\prec}{~\hat{<}~}
\newcommand\eqnCnt[1][]{ %
    \refstepcounter{subequation} %
    \begin{align}#1\end{align} %
    \addtocounter{equation}{-1}}
\def\mtabLong{long}
\makeatletter
\newenvironment{mtabular}[2][\empty]{ %
    \def\@xarraycr{ %
        \stepcounter{equation} %
        \setcounter{subequation}{0} %
        \@ifnextchar[\@argarraycr{\@argarraycr[\mtabskip]}}
    \let\theoldequation\theequation %
    \renewcommand\theequation{\theoldequation.\alph{subequation}}
    \edef\mtabOption{#1}
    \setcounter{subequation}{0} %
    \tabcolsep=0pt
    \ifx\mtabOption\mtabLong\longtable{#2}\else\tabular{#2}\fi %
}{ %
\ifx\mtabOption\mtabLong\endlongtable\else\endtabular\fi %
\let\theequation\theoldequation %
\stepcounter{equation}}
\makeatother

==> praemble/hft-macros-maths.tex <==
% Useful shortcuts
\newcommand{\mr}{\mathrm}
\newcommand{\ms}{\mathsf}
\newcommand{\mc}{\mathcal}
\newcommand{\wt}[1]{{\widetilde{#1}}}

% Matrices, vectors, operators: shortcuts
\newcommand{\veg}[1]{\bm{#1}}     % geometrical / physical vectors
\newcommand{\vet}[1]{\bm{ \mathfrak{#1}}}    % I used it for physical vectors with time-dependency
\newcommand{\mat}[1]{\mathsfbfit{#1}} % n x n-dimensional matrix
\newcommand{\uv}[1]{\hat{\veg{#1}}} % unit vectors
\renewcommand{\vec}[1]{\mathsfbfit{#1}} %n-dimensional vector
\newcommand{\wvec}[1]{\widetilde{\mathsfbfit{#1}}} %widetilde n-dimensional vector
\newcommand{\wmat}[1]{\widetilde{\mathsfbfit{#1}}} %widetilde n-dimensional vector
\newcommand{\op}[1]{\mathcal{#1}} % operator that takes a scalar-valued function
\newcommand{\vecop}[1]{\bm{\mathcal{#1}}} % operator that takes a vector-valued function
\newcommand{\mel}[1]{\mathsfit{#1}} 
\newcommand{\vel}[1]{\mathsfit{#1}}
\newcommand{\matel}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\vecel}[1]{\begin{bmatrix} #1 \end{bmatrix}}

% Special matrices
\newcommand{\matI}{\mathbfsf{I}}
\newcommand{\matO}{\mathbfsf{0}}
\newcommand{\vecO}{\matO}
\newcommand{\vecI}{\mathbfsf{1}}


% Special geometrical vectors (mainly normals and unit vectors etc.)
\newcommand{\n}{\hat{\bm{n}}} 
\newcommand{\un}{\hat{\bm{u}}}
\newcommand{\np}{\hat{\bm{n}}^\prime}  
\newcommand{\pn}{\partial_{\hat{\bm{n}}}} 
\newcommand{\pnp}{\partial_{\hat{\bm{n}}^\prime}}  
\newcommand{\pnnp}{\partial_{\hat{\bm{n}},\hat{\bm{n}}^\prime}}    
\newcommand{\hek}{\hat{\bm{e}}_k}

% Real and imaginary part
\renewcommand{\Re}{\mathrm{Re}\;}
\renewcommand{\Im}{\mathrm{Im}\;}

% Differential symbol
\newcommand{\dd}{\mathrm{d}}  % The differential symbol is actually an operator

% Differential fractions
\newcommand{\ntfrac}[2]{\frac{\nt{#1}}{\nt{#2}}}  % partielles Differential
\newcommand{\pfrac}[2]{\frac{\uppartial #1}{\uppartial #2}}  % partielles Differential
\newcommand{\fracpd}[2]{\frac{\uppartial #1}{\uppartial #2}} % partielles Differential
\newcommand{\fracppd}[2]{\frac{\uppartial^2 #1}{\uppartial #2^2}}  % zweite partielle 
\newcommand{\fracd}[2]{\frac{\dd#1}{\dd #2}} % partielles Differential
\newcommand{\fracdd}[2]{\frac{\dd^2 #1}{\dd#2^2}}  % zweite partielle 

% Imaginary unit
\newcommand{\ii}{\mathrm{i}}   % For mathematicians and backwards compatibility
\newcommand{\im}{\mathrm{i}}  % For mathematician, Julia notation
\newcommand{\jm}{\mathrm{j}}  % For engineer stuff 

% Other math constants
\newcommand{\e}{\mathrm{e}}
\newcommand{\ep}{\varepsilon}
\newcommand{\sg}{\varsigma}

% Blackboard font: for special sets
\newcommand{\bbone}{\mathds{1}}  % mathds benötigt das Package "dsfont"
%\newcommand{\C}{\mathbb{C}}
\newcommand{\B}{B}
\newcommand{\K}{\mathbb{K}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}

% Norms
%\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
%\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\newcommand{\pair}[2]{\langle #1, #2 \rangle}

% Math operators: analytic
\DeclareMathOperator{\hodge}{\mathbf{\upDelta}}
\DeclareMathOperator{\laplace}{\upDelta}
\DeclareMathOperator{\dirac}{\updelta}
\DeclareMathOperator{\dalembert}{\square}
\DeclareMathOperator{\ee}{e}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\tanc}{tanc}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\cond}{cond}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\Rang}{Rang}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Null}{null}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\tr}{trace}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Eig}{Eig}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\vcurl}{\mathbf{curl}}
\DeclareMathOperator{\besselJ}{J}
\DeclareMathOperator{\besselN}{N}
\DeclareMathOperator{\hankel}{H}
\DeclareMathOperator{\Ai}{Ai}
\DeclareMathOperator{\Bi}{Bi}
\DeclareMathOperator{\ricbessJ}{\mathbb{J}}
\DeclareMathOperator{\richankH}{\mathbb{H}}

% Math operators: linear algebra
\newcommand{\T}{\mr{T}}
\newcommand{\Ht}{\dagger}

% Math operators: special functions
\newcommand{\bJ}{\operatorname{J}}
\newcommand{\bH}{\operatorname{H}}
\newcommand{\bN}{\operatorname{N}}

% Math operation: restrain
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
        \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
        #1 % the function
        \vphantom{|} % pretend it's a little taller at normal size
        \right|_{#2} % this is the delimiter
}}


\newcommand\rst[3]{{% we make the whole thing an ordinary symbol
        \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
        #1 % the function
        \vphantom{|} % pretend it's a little taller at normal size
        \right|_{#2}^{#3} % this is the delimiter
}}

% Fourier transformations
\newcommand{\FT}{\cF}
\newcommand{\FTa}[1]{\cF\left[#1\right]}
\newcommand{\FTi}{\cF^{-1}}
\newcommand{\FTia}[1]{\cF^{-1}\left[#1\right]}

% Trace operators
\newcommand{\ttrace}{\upgamma_{\mathbf{t}}}
\newcommand{\Ntrace}{\upgamma_{\mathrm{N}}}

%
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

==> praemble/hft-macros.tex <==
\input{hft-macros-environments.tex} 
\input{hft-macros-maths.tex} 
\input{hft-packages-acro.tex} 
\input{hft-macros-booktabs.tex} 

% Other
\newcommand{\formatedtime}[3]{#1:#2:#3}
\newcommand{\formatedtimed}[4]{#1 days #2:#3:#4}

==> praemble/hft-packages-acro.tex <==
\usepackage{acro}

\DeclareAcronym{DG}
{
    short = DG ,
    long = discontinuous Galerkin
}


\DeclareAcronym{ACA}
{
    short = ACA ,
    long = adaptive cross approximation
}

\DeclareAcronym{EFIE}
{
    short =  EFIE ,
    long = electric field integral equation
}

\DeclareAcronym{MFIE}
{
    short =  MFIE ,
    long = magnetic field integral equation
}

\DeclareAcronym{CFIE}
{
    short =  CFIE ,
    long = combined field integral equation
}

\DeclareAcronym{MUIE}
{
    short =  MUIE ,
    long = Müller integral equation
}

\DeclareAcronym{PMCHWT}
{
    short =  PMCHWT ,
    long = Poggio-Miller-Chang-Harrington-Wu-Tsai integral equation
}

\DeclareAcronym{SPD}
{
    short =  SPD ,
    long = {symmetric, positive definite}
}

\DeclareAcronym{SPSD}
{
    short =  SPD ,
    long = {symmetric, positive semi-definite}
}

\DeclareAcronym{PEC}
{
    short =  PEC ,
    long = perfectly electrically conducting
}

\DeclareAcronym{RWG}
{
    short = RWG ,
    long = Rao-Wilton-Glisson
} 

\DeclareAcronym{BC}
{
    short = BC ,
    long = Buffa-Christiansen
} 


\DeclareAcronym{SVD}
{
    short = SVD ,
    long = singular value decomposition
} 


\DeclareAcronym{CG}
{
    short = CG ,
    long = conjugate gradient
} 

\DeclareAcronym{PCG}
{
    short = PCG ,
    long = preconditioned conjugate gradient
} 

\DeclareAcronym{CGS}
{
    short = CGS ,
    long = conjugate gradient squared
} 


\DeclareAcronym{CMP}
{
    short = CMP ,
    long = Calderón multiplicative preconditioner
} 

\DeclareAcronym{RFCMP}
{
    short = RF-CMP ,
    long = refinement-free Calderón multiplicative preconditioner
} 

\DeclareAcronym{HPD}
{
    short = HPD ,
    long = {Hermitian, positive definite}
} 

\DeclareAcronym{RHS}
{
    short = RHS ,
    long = {right-hand side}
}

\DeclareAcronym{PW}
{
    short = PW ,
    long = {plane wave}
} 

\DeclareAcronym{HD}
{
    short = HD ,
    long = {Hertzian dipole}
} 

\DeclareAcronym{FF}
{
    short = FF ,
    long = {far-field}
} 

\DeclareAcronym{NF}
{
    short = NF ,
    long = {near-field}
} 

==> praemble/hft-packages-cleveref.tex <==
\usepackage[english]{cleveref}

\Crefname{defn}{definition}{definitions}
\Crefname{defn}{Definition}{Definitions}

\Crefname{asm}{assumption}{assumptions}
\Crefname{asm}{Assumption}{Assumptions}

\crefname{lem}{lemma}{lemmas} 
\Crefname{lem}{Lemma}{Lemmas}

\crefname{prop}{proposition}{propositions} 
\Crefname{prop}{Proposition}{Propositions}

\crefname{thm}{theorem}{theorms} 
\Crefname{thm}{Theorem}{Theorms}

\crefname{cor}{corollary}{corollaries}
\Crefname{cor}{Corollary}{Corollaries}

==> praemble/hft-packages-review.tex <==
\usepackage{lineno}
\modulolinenumbers[5]
%\usepackage{todonotes}
\usepackage{umoline}

\newcommand{\td}[1]{\todo[inline,size=\small]{#1}} % inline todo notes

==> praemble/hft-packages-theorem.tex <==
%%% Configure AMS MATH
\theoremstyle{definition}
\newtheorem{defn}{Definition}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{prop}{Proposition}

\theoremstyle{remark}
\newtheorem*{remark}{Remark}


==> praemble/hft-packages-tikz-pgfplots.tex <==
\usepackage{pgfplots}
\usepackage{pgfplotstable}
% and optionally (as of Pgfplots 1.3):
\pgfplotsset{compat=newest}
\pgfplotsset{plot coordinates/math parser=false}
\newlength\figureheight
\newlength\figurewidth
\pgfplotsset{every axis plot/.append style={line width=1.5pt},
    legend style={font=\footnotesize, 
        text height=1.0ex,
        draw=black,
        fill=white,
        legend cell align=left}}


==> praemble/hft-paper-praemble-main.tex <==
\input{hft-paper-praemble-packages.tex}
\input{hft-macros.tex}
\input{sba-macros.tex}

==> praemble/hft-paper-praemble-packages.tex <==
% ill unnecessary alphabets
\newcommand{\hmmax}{0} 
\newcommand{\bmmax}{0} 

% Use UTF8
\usepackage[utf8]{luainputenc}

% Activate T1
\usepackage[T1]{fontenc}

\usepackage{graphicx}
% \usepackage[dvipsnames]{xcolor}

% Ensure that we are language aware
\usepackage[english]{babel}
\addto\captionsenglish{\renewcommand{\figurename}{Fig.}}
\addto\captionsenglish{\renewcommand{\tablename}{Tab.}}
\usepackage{csquotes}

% Font stuff
\usepackage{newtxtext}
\usepackage{amsthm}
\usepackage[slantedGreek]{newtxmath}
%\usepackage{mathsfbf}
\usepackage[OMLmathsfit]{isomath}
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}
\usepackage{bm}
% Math packages
\usepackage{envmath}
\usepackage{mathtools}
\usepackage{commath}
\usepackage{siunitx}
%\usepackage{IEEEtrantools}
%\usepackage{amssymb} % SA: This package conflicts with the other font packages

% Figures
\usepackage[caption=false,font=footnotesize]{subfig}


% Tables
\usepackage{booktabs}
\usepackage{footmisc}  % Footnotes in floating environments

% Other
\usepackage{url}

\input{hft-packages-theorem.tex}
\input{hft-packages-review.tex}
\input{hft-packages-tikz-pgfplots.tex}
%\input{hft-packages-acro.tex}
%\usepackage{hyperref} % Load before cleveref
\input{hft-packages-cleveref.tex}

==> praemble/sba-macros.tex <==
\NewDocumentCommand{\TA}{o}{
    \IfNoValueTF {#1} {%
        \vecop T_{\kern-2pt\mr{A}}
    }
    {
        \vecop T_{\kern-2pt\mr{A},#1}
    }
}

\NewDocumentCommand{\TPhi}{o}{
    \IfNoValueTF {#1} {%
        \vecop T_{\kern-2pt\Phiup}
    }
    {
        \vecop T_{\kern-2pt\Phiup,#1}
    }
}

\NewDocumentCommand{\matTA}{o}{
    \IfNoValueTF {#1} {%
        \mat T_\mr{A}   
        }
    {
        \mat T_{\mr{A},#1}
    }
}

\NewDocumentCommand{\matTPhi}{o}{
    \IfNoValueTF {#1} {%
        \mat T_\Phiup   
        }
    {
        \mat T_{\Phiup,#1}
    }
}

% Maxwell Single layer
\NewDocumentCommand{\MSL}{o}{
    \IfNoValueTF {#1} {%
        \veg \Psi_\mr{SL}
        }
    {
        \veg \Psi_{\mr{SL},#1}
    }
}

% Maxwell Double layer
\NewDocumentCommand{\MDL}{o}{
    \IfNoValueTF {#1} {%
        \veg \Psi_\mr{DL}
        }
    {
        \veg \Psi_{\mr{DL},#1}
    }
}

% vector Potential A
\NewDocumentCommand{\PA}{o}{
    \IfNoValueTF {#1} {%
        \veg \Psi_\mr{A}
        }
    {
        \veg \Psi_{\mr{A},#1}
    }
}

% Maxwell Double layer
\NewDocumentCommand{\PPhi}{o}{
    \IfNoValueTF {#1} {%
        \veg \Psi_{\Phiup}
        }
    {
        \veg \Psi_{\Phiup,#1}
    }
}


%\newcommand{\TA}{\vecop T_{\kern-4pt\mr{A}}}
%\newcommand{\TPhi}{\vecop T_{\kern-4pt\Phiup}}

%\newcommand{\matTA}{\mat T_\mr{A}}
%\newcommand{\matTPhi}{\mat T_\Phiup}

\newcommand{\ZA}{\mat{Z}_\ms{A}}    
\newcommand{\ZPhi}{\mat{Z}_\ms{\Phi}}    

\newcommand{\matL}{\mat{\Lambda}}   
\newcommand{\matS}{\mat{\Sigma}}

\newcommand{\matLT}{\widetilde{\mat{\Lambda}}}   
\newcommand{\matST}{\widetilde{\mat{\Sigma}}}

\newcommand{\matLr}{\mat{\Lambda}_\ms{r}}
\newcommand{\matSr}{\mat{\Sigma}_\ms{r}}

\newcommand{\Pl}{\mat P_{\upLambda}}
\newcommand{\Ps}{\mat P_{\upSigma}}
\newcommand{\Pds}{\mat P_{\wt \upSigma}}
\newcommand{\Ph}{\mat P_{\mr H}}
\newcommand{\Plh}{\mat P_{\upLambda   \mr H}}
\newcommand{\Psh}{\mat P_{\upSigma   \mr H}}
\newcommand{\Pwl}{\wmat P_{\upLambda}}
\newcommand{\Pws}{\wmat P_{\upSigma}}
\newcommand{\Pwh}{\mat P_{\mr H}}
\newcommand{\Pwsh}{\wmat P_{\upSigma  \mr H}}

\newcommand{\hveg}[1]{\hat{\veg{#1}}}
\newcommand{\wveg}[1]{\widetilde{\veg{#1}}}

